The Eval4NLP Shared Task on Explainable Quality Estimation: Overview and Results

In this paper, we introduce the Eval4NLP-2021shared task on explainable quality estimation. Given a source-translation pair, this shared task requires not only to provide a sentence-level score indicating the overall quality of the translation, but also to explain this score by identifying the words that negatively impact translation quality. We present the data, annotation guidelines and evaluation setup of the shared task, describe the six participating systems, and analyze the results. To the best of our knowledge, this is the first shared task on explainable NLP evaluation metrics. Datasets and results are available at https://github.com/eval4nlp/SharedTask2021.

==> BT_system_comparison.tex <==
\paragraph{Rigorous system comparison.}
Previous systems are ranked according to their global statistics such as \cpt{MEAN}, e.g., comparing averaged AUC scores of different systems over a common set of test instances. However, such aggregation mechanisms ignore which system beats which over instances, and thus come at the risk of producing false comparison results. For instance, \citet{bt:2021} find that a system worse than another on all instances but one (an outlier) might be falsely declared the winner according to \cpt{MEAN} (and \cpt{MEDIAN} also). As remedies, they suggest to use \cpt{BT} to perform rigorous comparison for competing systems. \cpt{BT} leverages instance-level paring of metric scores from different systems\footnote{\cpt{BT} is a statistical model used to maximize the likelihood of observed data—-which systems beats which on each instance, by which it estimates unknown, inherent strengths of systems. In the case of two systems, the strength of system A is equivalent to the percent of instances of A better than system B.}, and assume that a winning system should beat others over most of instances. 

Our preliminary study shows that \cpt{MEAN} and \cpt{BT} strongly disagree on SotA and Top-3 systems across language pairs and metrics; however, system rankings according to \cpt{BT} are not always trustworthy. To illustrate this, we show evidence for \cpt{BT} over \cpt{MEAN} and for that \cpt{BT} might be wrong as listed below:

\input{figures/bt_matrix}
\begin{itemize}

\item \cpt{BT} over \cpt{MEAN} (see Fig.~\ref{fig:bt}(left)): \cpt{MEAN} declares Kyoto-1 the best; however, it significantly outperforms merely 3 out of 9 systems according to pairwise comparison. This hints that \cpt{MEAN} results are very likely wrong. In contrast, \cpt{BT} chooses Unbabel-18 according to that it wins in 8 out of 9 cases. 

\item \cpt{BT} might be wrong (see Fig.~\ref{fig:bt}(right)): \cpt{BT} declares Unbabel-18 the best, as it beats 7 out of 10 systems with clear wins. On the other hand, Kyoto-1 (ranked at the 5th place according to \cpt{BT}) wins in 9 out of 10 systems (often by a small margin though), and it also beats Unbabel-18. This means Kyoto-1 might be the winner, given that \cpt{BT} yields a counter-intuitive judgment.
\end{itemize}

Overall, \cpt{BT} is more rigorous than \cpt{MEAN} to yield system rankings, as it bases its judgments on  pairwise comparison, i.e., judging how good a system is against others (judgments sometimes might be wrong, though). When one favors rigorous comparison of competing systems, there is no clear winner in the shared task, as as none of systems beats all other systems according to pairwise comparison.


==> figures/bt_matrix.tex <==
\begin{figure*}
\centering
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{figures/source.rec-topk_scores.de-zh.pdf}
\end{subfigure}
\begin{subfigure}[b]{0.49\textwidth}
\includegraphics[width=\textwidth]{figures/target.rec-topk_scores.de-zh.pdf}
\end{subfigure}
\caption{Results of pairwise comparison according to (left) source.rec-topk-scores and (right) target.rec-topk-scores over system pairs for German-to-Chinese. Each cell denotes the percent of the number of instances on which one system (in rows) beats another (in columns). We mark cells for which system pairs have significant differences according to Sign test. Systems have been ranked by BT, e.g., systems in final rows declare the best. \cpt{Mean} declares Kyoto-1 the best in both (left) and (right) settings.}
\label{fig:bt}
\end{figure*}


==> figures/data_example.tex <==
\begin{figure*}
\centering
\includegraphics[width=0.9\textwidth]{figures/data_example.png}
\caption{Example of the data collected for the Shared Task and the output expected from the participants.}
\label{fig:data_example}
\end{figure*}


==> figures/perc_tags.tex <==
\begin{figure}
\centering
\begin{subfigure}[b]{0.48\textwidth}
\includegraphics[width=\textwidth]{figures/perc_tags.png}
\end{subfigure}
\caption{Percentage of source and target tokens annotated as rationale for sentence-level ratings.}
\label{fig:dist_tags}
\end{figure}


==> figures/task_example.tex <==
\begin{figure}
\centering
\includegraphics[width=0.5\textwidth]{figures/task_example.png}
\caption{Example of the test data and the output expected from the participants.}
\label{fig:task_example}
\end{figure}


==> tables/agreement.tex <==
\begin{table}[!htb]
    \small
    \centering
    \begin{tabular}{c|ccc}
    \toprule
               &  \textbf{Sentence-Level} & \textbf{Word-Level} \\ \midrule
         De-Zh & 0.59 & 0.515 \\
         Ru-De & 0.71 & 0.575 \\
         Ro-En & 0.81 & 0.602 \\
         Et-En & 0.68 & 0.438 \\
         \bottomrule
    \end{tabular}
    \caption{Sentence-level (Pearson) and word-level (kappa) agreements for different language pairs.}
    \label{table:agreements}
\end{table}


==> tables/results_dezh.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{lcccc|cccc|c}
    \toprule
	& \multicolumn{4}{c|}{Target} & \multicolumn{4}{c|}{Source} & \multicolumn{1}{c}{Sentence}  \\
	& Rank & AUC & AP & Rec & Rank & AUC & AP & Rec & Pearson \\
    \midrule
    IST-Unbabel (2) & 2.3 & 0.68 & 0.50 & 0.37 & 3.0 & 0.67 & 0.47 & 0.32 & 0.33\\
    IST-Unbabel (1)* & 2.7 & 0.71 & 0.47 & 0.34 & 2.0 & 0.73 & 0.50 & 0.35 & 0.27\\
    CUNI Prague* & 4.3 & 0.61 & 0.44 & 0.30 & 5.0 & 0.62 & 0.42 & 0.27 & 0.25\\
    OsakaUNLP & 5.3 & 0.59 & 0.41 & 0.28 & 6.3 & 0.58 & 0.39 & 0.25 & 0.01\\
    CLIP-UMD & 5.3 & 0.63 & 0.40 & 0.27 & 7.0 & 0.61 & 0.31 & 0.25 & 0.50\\
    Gringham & 7.3 & 0.55 & 0.36 & 0.22 & 4.0 & 0.64 & 0.42 & 0.27 & -0.04\\
    Baseline: XMOVER-SHAP & 7.7 & 0.55 & 0.33 & 0.22 & 10.0 & 0.47 & 0.29 & 0.16 & 0.18\\
    HeyTUDa & 9.0 & 0.51 & 0.31 & 0.18 & 11.0 & -1.00 & -1.00 & -1.00 & 0.34\\
    Baseline: Random & 10.0 & 0.50 & 0.29 & 0.17 & 8.7 & 0.50 & 0.30 & 0.17 & 0.00\\
    Baseline: TransQuest-LIME & 11.0 & 0.46 & 0.27 & 0.14 & 8.0 & 0.49 & 0.32 & 0.20 & 0.34\\
    \bottomrule
\end{tabular}
\caption{Official results of the Eval4NLP Shared Task on Explainable Quality Estimation for German-Chinese. Submissions to the unconstrained track are marked with *. Submissions not significantly outperformed by any other submission for each metric are marked in bold.}
\label{tab:dezh-results}
\end{table*}


==> tables/results_eten.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{lcccc|cccc|c}
    \toprule
	& \multicolumn{4}{c|}{Target} & \multicolumn{4}{c|}{Source} & \multicolumn{1}{c}{Sentence}  \\
	& Rank & AUC & AP & Rec & Rank & AUC & AP & Rec & Pearson \\
	\midrule
	IST-Unbabel (1)* & 1.0 & \textbf{0.92} & \textbf{0.85} & \textbf{0.76} & 1.3 & \textbf{0.94} & \textbf{0.86} & \textbf{0.77} & 0.86\\
    CUNI Prague* & 2.0 & 0.92 & 0.84 & \textbf{0.75} & 3.0 & 0.93 & \textbf{0.85} & \textbf{0.76} & 0.80\\
    NICT Kyoto & 3.0 & \textbf{0.90} & 0.82 & \textbf{0.73} & 1.7 & 0.93 & 0.85 & \textbf{0.77} & 0.85\\
    IST-Unbabel (2) & 4.3 & 0.82 & 0.74 & 0.63 & 4.7 & 0.86 & 0.76 & 0.64 & 0.82\\
    Gringham & 5.0 & 0.84 & 0.71 & 0.60 & 6.0 & 0.86 & 0.72 & 0.59 & 0.71\\
%     OsakaUNLP & 5.7 & 0.82 & 0.71 & 0.61 & 4.3 & 0.87 & 0.76 & 0.65 & 0.65\\
    CLIP-UMD & 7.0 & 0.74 & 0.63 & 0.53 & 7.0 & 0.76 & 0.51 & 0.45 & 0.77\\
    Baseline: TransQuest-LIME & 8.3 & 0.62 & 0.54 & 0.43 & 8.0 & 0.54 & 0.44 & 0.31 & 0.77\\
    HeyTUDa & 8.7 & 0.66 & 0.52 & 0.41 & 11.0 & -1.00 & -1.00 & -1.00 & 0.77\\
    Baseline: XMOVER-SHAP & 10.0 & 0.62 & 0.44 & 0.34 & 9.0 & 0.54 & 0.37 & 0.23 & 0.49\\
    Baseline: Random & 11.0 & 0.50 & 0.36 & 0.25 & 10.0 & 0.49 & 0.34 & 0.19 & -0.03\\
    \bottomrule
\end{tabular}
\caption{Official results of the Eval4NLP Shared Task on Explainable Quality Estimation for Estonian-English. Submissions to the unconstrained track are marked with *. Submissions not significantly outperformed by any other submission for each metric are marked in bold.}
\label{tab:eten-results}
\end{table*}


==> tables/results_roen.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{lcccc|cccc|c}
    \toprule
	& \multicolumn{4}{c|}{Target} & \multicolumn{4}{c|}{Source} & \multicolumn{1}{c}{Sentence}  \\
	& Rank & AUC & AP & Rec & Rank & AUC & AP & Rec & Pearson \\
	\midrule
	NICT Kyoto & 1.0 & \textbf{0.95} & \textbf{0.87} & \textbf{0.78} & 1.0 & \textbf{0.95} & \textbf{0.85} & \textbf{0.75} & 0.92\\
    IST-Unbabel (1)* & 2.0 & 0.94 & 0.84 & 0.75 & 2.0 & 0.93 & 0.81 & 0.71 & 0.87\\
    CUNI Prague* & 3.0 & 0.94 & 0.83 & 0.73 & 3.0 & 0.93 & 0.81 & 0.70 & 0.89\\
    IST-Unbabel (2) & 4.0 & 0.88 & 0.78 & 0.68 & 5.0 & 0.86 & 0.73 & 0.62 & 0.90\\
%     OsakaUNLP & 5.0 & 0.87 & 0.76 & 0.67 & 4.0 & 0.89 & 0.75 & 0.64 & 0.76\\
    Gringham & 6.0 & 0.87 & 0.73 & 0.61 & 6.0 & 0.84 & 0.61 & 0.45 & 0.78\\
    CLIP-UMD & 7.0 & 0.73 & 0.60 & 0.49 & 7.0 & 0.72 & 0.41 & 0.37 & 0.90\\
    Baseline: TransQuest-LIME & 8.7 & 0.63 & 0.52 & 0.42 & 8.7 & 0.48 & 0.35 & 0.24 & 0.90\\
    HeyTUDa & 8.7 & 0.68 & 0.50 & 0.38 & 11.0 & -1.00 & -1.00 & -1.00 & 0.90\\
    Baseline: XMOVER-SHAP & 9.7 & 0.67 & 0.44 & 0.30 & 9.0 & 0.53 & 0.29 & 0.15 & 0.70\\
    Baseline: Random & 11.0 & 0.52 & 0.31 & 0.19 & 9.3 & 0.50 & 0.28 & 0.15 & 0.02\\
    \bottomrule
\end{tabular}
\caption{Official results of the Eval4NLP Shared Task on Explainable Quality Estimation for Romanian-English. Submissions to the unconstrained track are marked with *. Submissions not significantly outperformed by any other submission for each metric are marked in bold.}
\label{tab:roen-results}
\end{table*}


==> tables/results_rude.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{lcccc|cccc|c}
    \toprule
	& \multicolumn{4}{c|}{Target} & \multicolumn{4}{c|}{Source} & \multicolumn{1}{c}{Sentence}  \\
	& Rank & AUC & AP & Rec & Rank & AUC & AP & Rec & Pearson \\
    \midrule
    NICT Kyoto & 1.0 & \textbf{0.93} & \textbf{0.83} & \textbf{0.74} & 1.0 & \textbf{0.92} & \textbf{0.80} & \textbf{0.71} & 0.68\\
    IST-Unbabel (1)* & 2.0 & 0.80 & 0.64 & 0.52 & 2.0 & 0.85 & 0.71 & 0.59 & 0.67\\
    CUNI Prague* & 3.3 & 0.76 & 0.61 & 0.50 & 3.3 & 0.80 & 0.67 & 0.56 & 0.61\\
    Gringham & 4.3 & 0.79 & 0.57 & 0.46 & 3.7 & 0.84 & 0.67 & 0.56 & 0.60\\
    IST-Unbabel (2) & 4.3 & 0.75 & 0.58 & 0.47 & 5.7 & 0.77 & 0.63 & 0.52 & 0.64\\
    OsakaUNLP & 6.0 & 0.71 & 0.52 & 0.41 & 5.3 & 0.79 & 0.62 & 0.52 & 0.62\\
    CLIP-UMD & 7.0 & 0.65 & 0.46 & 0.36 & 7.3 & 0.66 & 0.41 & 0.37 & 0.30\\
    HeyTUDa & 8.3 & 0.54 & 0.33 & 0.23 & 11.0 & -1.00 & -1.00 & -1.00 & 0.50\\
    Baseline: XMOVER-SHAP & 8.7 & 0.52 & 0.33 & 0.23 & 9.0 & 0.52 & 0.36 & 0.26 & 0.25\\
    Baseline: Random & 10.0 & 0.49 & 0.31 & 0.22 & 10.0 & 0.51 & 0.34 & 0.24 & -0.02\\
    Baseline: TransQuest-LIME & 11.0 & 0.40 & 0.26 & 0.16 & 7.7 & 0.53 & 0.43 & 0.32 & 0.50\\
    \bottomrule
\end{tabular}
\caption{Official results of the Eval4NLP Shared Task on Explainable Quality Estimation for Russian-German. Submissions to the unconstrained track are marked with *. Submissions not significantly outperformed by any other submission for each metric are marked in bold.}
\label{tab:rude-results}
\end{table*}


==> tables/table_clf_results.tex <==
\begin{table*}[t]
\small
\centering
\begin{tabular}{lccccc}
\toprule
& Et-En & Ro-En & De-Zh & Ru-De \\
\midrule
NICT-Kyoto & 0.58 & 0.72 & 0.35 & 0.60 \\
IST-Unbabel-unconstr & 0.63 & 0.72 & 0.09 & 0.39 \\
CUNI & 0.61 & 0.69 & 0.00 & 0.36 \\
Gringham & 0.46 & 0.64 & 0.00 & 0.37 \\
OsakaUNLP & 0.42 & 0.68 & -0.00 & 0.26 \\
IST-Unbabel & 0.40 & 0.43 & 0.10 & 0.23 \\
Tasnim & 0.34 & 0.47 & 0.00 & 0.05 \\
TransQuest-LIME & 0.20 & 0.22 & 0.00 & 0.00 \\
HeyTUDa & 0.15 & 0.10 & 0.00 & 0.01 \\
XMOVER-SHAP & 0.02 & 0.16 & 0.00 & 0.00 \\
Random & 0.00 & 0.00 & 0.00 & 0.00 \\
\bottomrule
\end{tabular}
\caption{MCC results for a logistic regression classifier fitted with 5-fold cross-validation on the testset}
\label{tab:rude-results}
\end{table*}

